A note on complex plane curve singularities up to diffeomorphism and their rigidity

We prove that, if two germs of plane curves $(C,0)$ and $(C',0)$ with at least one singular branch are equivalent by a (real) smooth diffeomorphism, then $C$ is complex isomorphic to $C'$ or to $\overline{C'}$. A similar result was shown by Ephraim for irreducible hypersurfaces before, but his proof is not constructive. Indeed, we show that the complex isomorphism is given by the Taylor series of the diffeomorphism. We also prove an analogous result for the case of non-irreducible hypersurfaces containing an irreducible component of zero-dimensional isosingular locus. Moreover, we provide a general overview of the different classifications of plane curve singularities.

==> Style-and-more.tex <==
% Use \input{Style-and-more} to embed this text in your LaTeX file (this is as if you wrote everything that is here)
% See https://tex.stackexchange.com/questions/246/when-should-i-use-input-vs-include?noredirect=1&lq=1

%Usual type of document:
%\documentclass[a4paper,12pt]{amsart}
%\documentclass[a4paper,11pt]{book}

\binoppenalty=9999
\relpenalty=9999% for better linebraeks in math mode https://tex.stackexchange.com/questions/10850/stop-latex-from-breaking-an-inline-math-equation

%\newcommand{\name}{action}

\def\im{\operatorname{im}}
\def\dim{\operatorname{dim}}
\def\deg{\operatorname{deg}}
\def\bideg{\operatorname{bideg}}
\def\rank{\operatorname{rank}}
\def\rk{\operatorname{rank}}
\def\corank{\operatorname{corank}}
\def\coker{\operatorname{coker}}
\def\codim{\operatorname{codim}}
\def\ind{\operatorname{ind}}
\def\id{\operatorname{id}}
\def\Id{\operatorname{id}}
\def\ord{\operatorname{ord}}
\def\Re{\operatorname{Re}}
\def\Im{\operatorname{Im}}
\def\sign{\operatorname{sgn}}
\def\sgn{\operatorname{sgn}}
\def\Span{\operatorname{Span}}
\def\Bihol{\operatorname{Bihol}}
\def\Diff{\operatorname{Diff}}
\def\tr{\operatorname{tr}}
\def\rhd{\operatorname{rhd}}

\newcommand{\Alt}{\textnormal{Alt}}
\newcommand{\RR}{\mathbb{R}}
\newcommand{\KK}{\mathbb{K}}
\newcommand{\CC}{\mathbb{C}}
\newcommand{\QQ}{\mathbb{Q}}
\newcommand{\ZZ}{\mathbb{Z}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\K}{\mathbb{K}}
\newcommand{\C}{\mathbb{C}}
\newcommand{\Q}{\mathbb{Q}}
\newcommand{\Z}{\mathbb{Z}}
\newcommand{\N}{\mathbb{N}}

\newcommand{\eqA}{\mathscr{A}}
\newcommand{\eqK}{\mathscr{K}}
\newcommand{\idm}{\mathfrak{m}}
\newcommand{\OO}{\mathcal{O}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\Ascr}{\mathscr{A}}
\newcommand{\Bscr}{\mathscr{B}}
\newcommand{\Cscr}{\mathscr{C}}
\newcommand{\Dscr}{\mathscr{D}}
\newcommand{\Escr}{\mathscr{E}}
\newcommand{\Fscr}{\mathscr{F}}
\newcommand{\Gscr}{\mathscr{G}}
\newcommand{\Hscr}{\mathscr{H}}
\newcommand{\Iscr}{\mathscr{I}}
\newcommand{\Jscr}{\mathscr{J}}
\newcommand{\Kscr}{\mathscr{K}}
\newcommand{\Lscr}{\mathscr{L}}
\newcommand{\Mscr}{\mathscr{M}}
\newcommand{\Nscr}{\mathscr{N}}
\newcommand{\Oscr}{\mathscr{O}}
\newcommand{\Pscr}{\mathscr{P}}
\newcommand{\Qscr}{\mathscr{Q}}
\newcommand{\Rscr}{\mathscr{R}}
\newcommand{\Sscr}{\mathscr{S}}
\newcommand{\Tscr}{\mathscr{T}}
\newcommand{\Uscr}{\mathscr{U}}
\newcommand{\Vscr}{\mathscr{V}}
\newcommand{\Wscr}{\mathscr{W}}
\newcommand{\Xscr}{\mathscr{X}}
\newcommand{\Yscr}{\mathscr{Y}}
\newcommand{\Zscr}{\mathscr{Z}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\abf}{\mathbf{a}}
\newcommand{\bbf}{\mathbf{b}}
\newcommand{\cbf}{\mathbf{c}}
\newcommand{\dbf}{\mathbf{d}}
\newcommand{\ebf}{\mathbf{e}}
\newcommand{\fbf}{\mathbf{f}}
\newcommand{\gbf}{\mathbf{g}}
\newcommand{\hbf}{\mathbf{h}}
\newcommand{\ibf}{\mathbf{i}}
\newcommand{\jbf}{\mathbf{j}}
\newcommand{\kbf}{\mathbf{k}}
\newcommand{\lbf}{\mathbf{l}}
\newcommand{\mbf}{\mathbf{m}}
\newcommand{\nbf}{\mathbf{n}}
\newcommand{\obf}{\mathbf{o}}
\newcommand{\pbf}{\mathbf{p}}
\newcommand{\qbf}{\mathbf{q}}
\newcommand{\rbf}{\mathbf{r}}
\newcommand{\sbf}{\mathbf{s}}
\newcommand{\tbf}{\mathbf{t}}
\newcommand{\ubf}{\mathbf{u}}
\newcommand{\vbf}{\mathbf{v}}
\newcommand{\wbf}{\mathbf{w}}
\newcommand{\xbf}{\mathbf{x}}
\newcommand{\ybf}{\mathbf{y}}
\newcommand{\zbf}{\mathbf{z}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\Abf}{\mathbf{A}}
\newcommand{\Bbf}{\mathbf{B}}
\newcommand{\Cbf}{\mathbf{C}}
\newcommand{\Dbf}{\mathbf{D}}
\newcommand{\Ebf}{\mathbf{E}}
\newcommand{\Fbf}{\mathbf{F}}
\newcommand{\Gbf}{\mathbf{G}}
\newcommand{\Hbf}{\mathbf{H}}
\newcommand{\Ibf}{\mathbf{I}}
\newcommand{\Jbf}{\mathbf{J}}
\newcommand{\Kbf}{\mathbf{K}}
\newcommand{\Lbf}{\mathbf{L}}
\newcommand{\Mbf}{\mathbf{M}}
\newcommand{\Nbf}{\mathbf{N}}
\newcommand{\Obf}{\mathbf{O}}
\newcommand{\Pbf}{\mathbf{P}}
\newcommand{\Qbf}{\mathbf{Q}}
\newcommand{\Rbf}{\mathbf{R}}
\newcommand{\Sbf}{\mathbf{S}}
\newcommand{\Tbf}{\mathbf{T}}
\newcommand{\Ubf}{\mathbf{U}}
\newcommand{\Vbf}{\mathbf{V}}
\newcommand{\Wbf}{\mathbf{W}}
\newcommand{\Xbf}{\mathbf{X}}
\newcommand{\Ybf}{\mathbf{Y}}
\newcommand{\Zbf}{\mathbf{Z}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\Abb}{\mathbb{A}}
\renewcommand{\Bbb}{\mathbb{B}}
\newcommand{\Cbb}{\mathbb{C}}
\newcommand{\Dbb}{\mathbb{D}}
\newcommand{\Ebb}{\mathbb{E}}
\newcommand{\Fbb}{\mathbb{F}}
\newcommand{\Gbb}{\mathbb{G}}
\newcommand{\Hbb}{\mathbb{H}}
\newcommand{\Ibb}{\mathbb{I}}
\newcommand{\Jbb}{\mathbb{J}}
\newcommand{\Kbb}{\mathbb{K}}
\newcommand{\Lbb}{\mathbb{L}}
\newcommand{\Mbb}{\mathbb{M}}
\newcommand{\Nbb}{\mathbb{N}}
\newcommand{\Obb}{\mathbb{O}}
\newcommand{\Pbb}{\mathbb{P}}
\newcommand{\Qbb}{\mathbb{Q}}
\newcommand{\Rbb}{\mathbb{R}}
\newcommand{\Sbb}{\mathbb{S}}
\newcommand{\Tbb}{\mathbb{T}}
\newcommand{\Ubb}{\mathbb{U}}
\newcommand{\Vbb}{\mathbb{V}}
\newcommand{\Wbb}{\mathbb{W}}
\newcommand{\Xbb}{\mathbb{X}}
\newcommand{\Ybb}{\mathbb{Y}}
\newcommand{\Zbb}{\mathbb{Z}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\Afrak}{\mathfrak{A}}
\newcommand{\Bfrak}{\mathfrak{B}}
\newcommand{\Cfrak}{\mathfrak{C}}
\newcommand{\Dfrak}{\mathfrak{D}}
\newcommand{\Efrak}{\mathfrak{E}}
\newcommand{\Ffrak}{\mathfrak{F}}
\newcommand{\Gfrak}{\mathfrak{G}}
\newcommand{\Hfrak}{\mathfrak{H}}
\newcommand{\Ifrak}{\mathfrak{I}}
\newcommand{\Jfrak}{\mathfrak{J}}
\newcommand{\Kfrak}{\mathfrak{K}}
\newcommand{\Lfrak}{\mathfrak{L}}
\newcommand{\Mfrak}{\mathfrak{M}}
\newcommand{\Nfrak}{\mathfrak{N}}
\newcommand{\Ofrak}{\mathfrak{O}}
\newcommand{\Pfrak}{\mathfrak{P}}
\newcommand{\Qfrak}{\mathfrak{Q}}
\newcommand{\Rfrak}{\mathfrak{R}}
\newcommand{\Sfrak}{\mathfrak{S}}
\newcommand{\Tfrak}{\mathfrak{T}}
\newcommand{\Ufrak}{\mathfrak{U}}
\newcommand{\Vfrak}{\mathfrak{V}}
\newcommand{\Wfrak}{\mathfrak{W}}
\newcommand{\Xfrak}{\mathfrak{X}}
\newcommand{\Yfrak}{\mathfrak{Y}}
\newcommand{\Zfrak}{\mathfrak{Z}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\afrak}{\mathfrak{a}}
\newcommand{\bfrak}{\mathfrak{b}}
\newcommand{\cfrak}{\mathfrak{c}}
\newcommand{\dfrak}{\mathfrak{d}}
\newcommand{\efrak}{\mathfrak{e}}
\newcommand{\ffrak}{\mathfrak{f}}
\newcommand{\gfrak}{\mathfrak{g}}
\newcommand{\hfrak}{\mathfrak{h}}
\newcommand{\ifrak}{\mathfrak{i}}
\newcommand{\jfrak}{\mathfrak{j}}
\newcommand{\kfrak}{\mathfrak{k}}
\newcommand{\lfrak}{\mathfrak{l}}
\newcommand{\mfrak}{\mathfrak{m}}
\newcommand{\nfrak}{\mathfrak{n}}
\newcommand{\ofrak}{\mathfrak{o}}
\newcommand{\pfrak}{\mathfrak{p}}
\newcommand{\qfrak}{\mathfrak{q}}
\newcommand{\rfrak}{\mathfrak{r}}
\newcommand{\sfrak}{\mathfrak{s}}
\newcommand{\tfrak}{\mathfrak{t}}
\newcommand{\ufrak}{\mathfrak{u}}
\newcommand{\vfrak}{\mathfrak{v}}
\newcommand{\wfrak}{\mathfrak{w}}
\newcommand{\xfrak}{\mathfrak{x}}
\newcommand{\yfrak}{\mathfrak{y}}
\newcommand{\zfrak}{\mathfrak{z}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\Acal}{\mathcal{A}}
\newcommand{\Bcal}{\mathcal{B}}
\newcommand{\Ccal}{\mathcal{C}}
\newcommand{\Dcal}{\mathcal{D}}
\newcommand{\Ecal}{\mathcal{E}}
\newcommand{\Fcal}{\mathcal{F}}
\newcommand{\Gcal}{\mathcal{G}}
\newcommand{\Hcal}{\mathcal{H}}
\newcommand{\Ical}{\mathcal{I}}
\newcommand{\Jcal}{\mathcal{J}}
\newcommand{\Kcal}{\mathcal{K}}
\newcommand{\Lcal}{\mathcal{L}}
\newcommand{\Mcal}{\mathcal{M}}
\newcommand{\Ncal}{\mathcal{N}}
\newcommand{\Ocal}{\mathcal{O}}
\newcommand{\Pcal}{\mathcal{P}}
\newcommand{\Qcal}{\mathcal{Q}}
\newcommand{\Rcal}{\mathcal{R}}
\newcommand{\Scal}{\mathcal{S}}
\newcommand{\Tcal}{\mathcal{T}}
\newcommand{\Ucal}{\mathcal{U}}
\newcommand{\Vcal}{\mathcal{V}}
\newcommand{\Wcal}{\mathcal{W}}
\newcommand{\Xcal}{\mathcal{X}}
\newcommand{\Ycal}{\mathcal{Y}}
\newcommand{\Zcal}{\mathcal{Z}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%



%\newcommand{\QED}{\qed\vspace{3mm}}

\newcommand{\RRzero}[1]{(\mathbb{R}^{#1},0)}
\newcommand{\CCzero}[1]{(\mathbb{C}^{#1},0)}
\newcommand{\RRS}[1]{(\mathbb{R}^{#1},S)}
\newcommand{\CCS}[1]{(\mathbb{C}^{#1},S)}
\newcommand{\GS}[2]{(\mathbb{C}^{#1},S)\rightarrow(\mathbb{C}^{#2},0)}
\newcommand{\Gzero}[2]{(\mathbb{C}^{#1},0)\rightarrow(\mathbb{C}^{#2},0)}
\newcommand{\Rzero}[1]{(\mathbb{R}^{#1},0)}
\newcommand{\Czero}[1]{(\mathbb{C}^{#1},0)}
\newcommand{\RS}[1]{(\mathbb{R}^{#1},S)}
\newcommand{\CS}[1]{(\mathbb{C}^{#1},S)}
\newcommand{\GSR}[2]{(\mathbb{R}^{#1},S)\rightarrow(\mathbb{R}^{#2},0)}
\newcommand{\GzeroR}[2]{(\mathbb{R}^{#1},0)\rightarrow(\mathbb{R}^{#2},0)}
%
\newcommand{\mdash}{\nobreakdash-\hspace{0pt}}%For the dash between maths-normalword and do properly the line breaks
\newcommand{\icss}{\textsc{icss} }

\newcommand{\cat}{%
	\mathbf%
}
\newcommand{\catop}[1]{%
	\cat{#1^\textrm{op}}%
}%

\newcommand{\toup}[1]{%
	\stackrel{#1}{\longrightarrow}%
}%
\newcommand{\todown}[1]{%
	\underset{#1}{\longrightarrow}%
}%

\newcommand{\barbelow}[1]{\underaccent{\bar}{#1}}
\newcommand{\transv}{\mathrel{\text{\tpitchfork}}}
\makeatletter
\newcommand{\tpitchfork}{%
  \vbox{
    \baselineskip\z@skip
    \lineskip-.52ex
    \lineskiplimit\maxdimen
    \m@th
    \ialign{##\crcr\hidewidth\smash{$-$}\hidewidth\crcr$\pitchfork$\crcr}
  }%
}
\makeatother

%This is to mimic a button in the pdf document, as in my thesis
%\newcommand*\keystroke[1]{%
  %\tikz[baseline=(key.base)]
    %\node[%
      %draw,
      %fill=white,
      %drop shadow={shadow xshift=0.25ex,shadow yshift=-0.25ex,fill=black,opacity=0.75},
      %rectangle,
      %rounded corners=2pt,
      %inner sep=1pt,
      %line width=0.5pt,
      %font=\scriptsize\sffamily
    %](key) {#1\strut}
  %;
%}




\theoremstyle{plain}
\newtheorem{theorem}{Theorem}[section]
\newtheorem*{theorem*}{Theorem}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem*{lemma*}{Lemma}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem*{corollary*}{Corollary}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{question}[theorem]{Question}
\newtheorem{thm}{Theorem}[section]
\newtheorem{lem}[theorem]{Lemma}
\newtheorem{cor}[theorem]{Corollary}
\newtheorem{prop}[theorem]{Proposition}
%\newtheorem*{falsetheorem}{\textsl{Generic theorem of spectral sequences}}
%\newtheorem*{falsetheoremm}{\textsl{Generic theorem of \textsc{icss}}}



\theoremstyle{definition}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{proposition/definition}[theorem]{Proposition/Definition}
\newtheorem{conjecture}[theorem]{Conjecture}
\newtheorem{example}[theorem]{Example}
\newtheorem{oproblem}[theorem]{Open Problem}
\newtheorem{remark}[theorem]{Remark}
\newtheorem{notation}[theorem]{Notation}
%\crefname{notation}{notation}{notations}
\Crefname{notation}{Notation}{Notations}

\theoremstyle{remark}
\newtheorem*{note}{Note}
\newtheorem{case}{Case}




% There is nothing compiling below this, only notes and stuff

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%.......%%%%.....%%%%%.......%%%%%%.....%%%.%%%..%%%....%%%%%
%%%%%%%.%%%%%%%.%%%%.%%%%%%%.%%%%%%%%.%%%%%%%%.%..%%%%.%%%%%%%%%
%%%%%%%.%%%%%%%.%%%.%%%%%%%%.%%%%%%%.%%%%%%%%%..%%%%%%%..%%%%%%%
%%%%%%%.%%%%%%%....%%%%%%%%%.%%%%%%%.%%%%%%%%%..%%%%%%%%%..%%%%%
%%%%%%%.%%%%%%%.%%%.%%%%%%%%.%%%%%%%%.%%%%%%%%.%..%%%%%%%%%.%%%%
%%%%%%%.%%%%%%%.%%%%.%%%%.......%%%%%%.....%%%.%%%..%%%....%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%Symbols en http://latex.wikia.com/wiki/List_of_LaTeX_symbols
%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%\setcounter{tocdepth}{1} for table of contents: 0 means only chapters, 1 includes sections, 2 includes subsections, etc.
%%\tableofcontents
%%\listoffigures
%%\listoftables
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%\usepackage{cellspace}%This is to add space in tables, when a specific column needs more space between rows, write an S before the text  https://tex.stackexchange.com/questions/247090/how-to-add-vertical-space-after-hline-without-breaking-vertical-lines-in-a-tabl/247096
%%\setlength\cellspacetoplimit{5pt}
%%\setlength\cellspacebottomlimit{5pt}

%%\usepackage[margin=0.6cm]{geometry}%To change every margin at once

%%\usepackage{enumitem}%To do several things in enumerate https://osl.ugr.es/CTAN/macros/latex/contrib/enumitem/enumitem.pdf

%\usepackage{amsmath,amsthm,amsfonts,amssymb,mathtools,mathrsfs}%Several symbols

%%\usepackage[spanish,es-lcroman]{babel}%Para usar latex como escribiendo en español. es-lcroman es para que no peten los enumerate en minúsculas con romanos ADEMÁS SI HAY FIGURAS CUYA RUTA TIENE ESPACIOS NO VALE CON HACER {``''} PORQUE DA PROBLEMAS CON ESPAŃOL, HAY QUE PONERLO EN INGLÉS Y HABRÁ QUE UQITAR TODO LO DE ADDTOSPANISH
%%\unaccentedoperators%Para no poner tildes en \lim

%%\usepackage{accents}%This is for barbelow

%%\usepackage{nicefrac}%For nice fractions in-text

%%\usepackage{diagbox}%To draw a diagonal in a box of a table ( https://ctan.math.illinois.edu/macros/latex/contrib/diagbox/diagbox.pdf )
%%\usepackage{makecell}%For several rows in a cell of a table (https://ctan.javinator9889.com/macros/latex/contrib/makecell/makecell.pdf)

%\usepackage{tikz-cd}% tikz-cd>graphicx, for commutative diagrams and such: http://ctan.math.washington.edu/tex-archive/graphics/pgf/contrib/tikz-cd/tikz-cd-doc.pdf
%\usetikzlibrary{babel}%Para que no haya problemas con símbolos y tikz\usepackage[shortlabels]{enumitem}%Para las opciones de enumerate como [(i)], shortlabels es para escribir i en lugar de [label={\upshape(\roman*)}] etc.  https://en.wikibooks.org/wiki/LaTeX/List_Structures https://tex.stackexchange.com/questions/100521/enumerate-inside-a-theorem-environment

%\usepackage[latin1]{inputenc}%Input encoding

%\usepackage[T1]{fontenc}%Font encoding (accents and umlauts and...)

%\usepackage{float}

%%\usepackage{mathdots}%For inverted diagonal points /   write \iddots

%%\usepackage{xcolor}% xcolor>color
%%\definecolor{colordelink}{rgb}{0,0,0.50}
%%\definecolor{colordecite}{rgb}{0,0.5,0}
%%\definecolor{colordeurl}{rgb}{0,0.41,0.5}

%%\usepackage[pagebackref=true]{hyperref}% To link references. COMPILE IN PDF!!!
%https://tex.stackexchange.com/questions/50747/options-for-appearance-of-links-in-hyperref
%%\hypersetup{
    %%colorlinks=true,
    %%linkcolor=colordelink,
    %%citecolor=colordecite,
		%%urlcolor=colordeurl,
		%%%,final%final option is to make it work with draft
%%}
%%\hypersetup{hidelinks}%Hides link rectangles

%%\usepackage[capitalize,nameinlink,noabbrev]{cleveref}% to emulate \autoref style

%%\usepackage[all]{hypcap}% for good href with figures https://tex.stackexchange.com/questions/27096/href-to-an-image-label-how-to-jump-to-the-image-instead-of-the-caption-below-t

%%\usepackage{subfigure}

%%\usepackage{multirow}

%%\usepackage{biblatex}%Gives problems

%\usepackage[nottoc]{tocbibind}%To make references appear in index

%\usepackage{todonotes}

%\usepackage{adjustbox}

%\usepackage[11pt]{moresize}

%\usepackage{epigraph}

%\decimalpoint%Necesario en español


%%\bibliographystyle{plain}
%%\bibliographystyle{abbrv}

%%\addto{\captionsspanish}{\renewcommand{\figurename}{Figure}}
%%\addto{\captionsspanish}{\renewcommand{\tablename}{Table}}
%%\addto{\captionsspanish}{\renewcommand{\bibname}{Bibliography}} %Para cambiar la palabra Referencias
 


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%A file %%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\begin{document}
%\author{R. Giménez Conejero
%D. Mond}
%
%\title[Title]
%{Title}
%
%
%
%\address{%Departament de Matemŕtiques,
%%Universitat de Val\`encia, Campus de Burjassot, 46100 Burjassot
%%SPAIN
%Alfr\'ed R\'enyi Institute of Mathematics, Re\'altanoda utca 13-15,
%H-1053 Budapest, 
%Hungary
%}
%\email{Roberto.Gimenez@uv.es}
%
%%\thanks{Work partially supported by MICINN Grant PGC2018--094889--B--I00 and by GVA Grant AICO/2019/024}
%
%\subjclass[2000]{Primary 58K15; Secondary 58K40, 58K65} \keywords{Deformations of map germs, homology, excellent unfoldings, coalescence, isotypes}
%
%
%\begin{abstract} 
%Abstract
%\end{abstract}
%
%
%\maketitle
%\section{Introduction}
%
%$\mathcal{a}$
%
%\emph{Acknowledgements:}
%...
%
%
%
%
%\bibliographystyle{abbrv}
%\bibliography{FullBib} % En el documento hay que poner acentos y m´yúsculas así: {M}ay\'uscul\^as
%\end{document}

%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%EJEMPLOS TIPO
%%\begin{align*} %To multiple-row equation
%%
%%y_{i+1} &= y_i + h f(y_{i+1}, t_i +h) \\
%%
%%y_{i+1} &= y_i + h \lambda y_{i+1} + g(t_i+h) 
%%
%%\end{align*}
%
%%To show only one number centered in align (https://tex.stackexchange.com/questions/13396/how-to-get-only-one-vertically-centered-equation-number-in-align-environment-with/17483#17483)
%%\begin{align}
  %%E_1&=A+B \label{eq:1}\\
   %%\begin{split}
    %%E_2&=(C-D)E_1 \label{eq:2}\\
    %%&\quad +[(1-R)+R(1-Y)\\
    %%&\quad +\pi(1-\delta)]E_2\\
    %%&\quad +F\cdot E_3
   %%\end{split}\\
  %%E_3 &=(\pi\cdot \chi)-(R\cdot E_1)-(RY\delta\cdot E_2) \label{eq:3}
%%\end{align}
%
%%\begin{table}[H]
%%	\centering
%%		\begin{tabular}{cc}
%%\includegraphics[width=0.55\textwidth]{C:/Users/Propietario/Desktop/P6/ImagenesEPS/f1eitodas.eps}&\includegraphics[width=0.55\textwidth]{C:/Users/Propietario/Desktop/P6/ImagenesEPS/f1eitodasampliado.eps}\\
%%				Aproximación de la primera función & Ampliación, detalle
%%		\end{tabular}
%%	\caption{}
%%	\label{tab:bla}
%%\end{table}
%%%%%%%%Para que la ruta de la imagen pueda tener espacios usar\includegraphics[width=1.00\textwidth]{{"C:/Users/rgc19/Desktop/TFM/Images/C2C3"}.png}  Y si la extensión no es eps. compilar dvi luego pdf
%
%
%%
%%Para una ecuación con un único número pero la ecuación está partida en dos:
%%\begin{equation}
%%\begin{aligned}
%%\beta_{k+1}(f)-\beta_k(f)=&\sum_{i\geq2} \frac{\textnormal{dim}\left(H(D^{k+i}(\tilde{f}))\right)^{[2,1,\dots,1]}}{i}-\mu(D^k(f))\\
%%&+\mu(D^{k+1}(f))-\textnormal{dim} H^{\Alt_2}(D^{k+1}(\tilde{f})).
%%\label{eq:betis}
%%\end{aligned}
%%\end{equation}
%
%
%%\[\mathcal{A} = \left(
%%\begin{tabular}{c c c c c}
%%$-2$  & $1$   &  $0 $   &$\cdots$  &  $0$ \\
%%$1$    & $-2$ & $1    $  &$\cdots$ &$  0 $\\
%%$0$    & $1$ &  $\ddots $&$\ddots$&$ \vdots$ \\
%%$\vdots$&$ \ddots$&$ \ddots$&$\cdots$&$ \vdots$\\
%%$0    $&  $ \cdots $&$\cdots$& $1 $&  $-2$\\
%%\end{tabular} \right)
%%\]
%
%%\begin{table}[H]
	%%\centering
		%%\begin{tabular}{|c||c|c|c|c|}
		%%\hline
				%%\multirow{2}{4em}{$E_M/E_{2M}$} & \multicolumn{2}{|c|}{$k=0.49h^2$}                     & \multicolumn{2}{|c|}{$k=0.01h$}\\ \cline{2-5}
								                  %%&  $l=1$                         &  $l=5$               &  $l=1$                         &  $l=5$           \\ \hline \hline
%%$M=24$                     &  $ 4.0290$ &  $3.8513$ &  $4.0400$ &  $4.1279$\\ \hline
%%$M=49$                     &  $ 4.0172$ &  $3.9731$ &  $ 4.0200$ &  $4.0418$\\ \hline
%%$M=99$                     &  $ 4.0092$ &  $3.9976$ &  $ 4.0100$ &  $4.0154$\\ \hline
%%$M=199$                   &  $ 4.0048$ &  $4.0018$ &  $ 4.0050$ &  $4.0063$\\ \hline
		%%\end{tabular}
%%\caption{Orden de Crank-Nicholson para $k=0.49h^2,0.01h$ y $l=1,5$}
%%\end{table}
%%%%%%%%%%%%%%%%%%%%%%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%INFO VARIA
%%http://www.latextemplates.com/
%%https://www.sharelatex.com?r=ce9db27b&rm=d&rs=b
%%http://gaussianos.com/chulatex-la-mejor-manera-de-llamar-a-una-chuleta-de-latex-y-otra-de-regalo/
%%http://web.mit.edu/rsi/www/pdfs/theorems.pdf
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%PARA HACER ECUACIONES MÁS GRANDES:
%%\[\scalebox{1.25}{$\mu_I(f,S)<\mu_I(\left\{f,g\right\},S\sqcup z)$} \]
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%%\setlength{\parindent}{4em} %para sangría
%%\setlength{\parskip}{1em}%para espaciado entre párrafos
%
%%\pushQED{\qed} 
%%a=b\qedhere
%%\popQED%https://tex.stackexchange.com/questions/66152/pushing-qed-to-the-right-within-a-displayed-formula
%
%\begin{document}
%
%\title{ Monodromy of germs of analytic functions }
%\date{  }
%\author{ Roberto Giménez Conejero, Universitat de Valčncia}
%\maketitle
%%%%%%%%%%%
%
%In this work we prove that, given $f:(X,x)\rightarrow (\mathbb{C}, 0)$ such that $f\in\mathfrak{M}^2O_ {X,x}$, there is a geometric local monodromy of $f$ without fixed points.

%\bibliographystyle{abbrv}
%\bibliographystyle{C:/Users/rgc19/AppData/Local/Programs/MiKTeX/bibtex/bst/bibtex/myalpha.bst}%https://tex.stackexchange.com/questions/168936/bibliography-style-merging-the-alpha-style-with-the-style-of-abbrv-for-author-i
%C:\Users\rgc19\AppData\Local\Programs\MiKTeX\bibtex\bst\bibtex\myalpha.bst
%\bibliography{FullBib} % En el documento hay que poner acentos y m´yúsculas así: {M}ay\'uscul\^as
%\bibliography{C:/Users/rgc19/Documents/Textos-Matematicas/Bibliografias/bibtex/bib/mybibs/FullBib.bib}
%%\bibliographystyle{plain}
%%\bibliography{Equising} % En el documento hay que poner acentos y m´yúsculas así: {M}ay\'uscul\^as
%\end{document}






